TPDiff: Temporal Pyramid Video Diffusion Model

The development of video diffusion models unveils a significant challenge: the substantial computational demands. To mitigate this challenge, we note that the reverse process of diffusion exhibits an inherent entropy-reducing nature. Given the inter-frame redundancy in video modality, maintaining full frame rates in high-entropy stages is unnecessary. Based on this insight, we propose TPDiff, a unified framework to enhance training and inference efficiency. By dividing diffusion into several stages, our framework progressively increases frame rate along the diffusion process with only the last stage operating on full frame rate, thereby optimizing computational efficiency. To train the multi-stage diffusion model, we introduce a dedicated training framework: stage-wise diffusion. By solving the partitioned probability flow ordinary differential equations (ODE) of diffusion under aligned data and noise, our training strategy is applicable to various diffusion forms and further enhances training efficiency. Comprehensive experimental evaluations validate the generality of our method, demonstrating 50% reduction in training cost and 1.5x improvement in inference efficiency.

==> fig/stage_diffusion.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/images/StageDiffusion_v2.pdf}
    % \vspace{-1em}
    \caption{\textit{\textbf{Stage-wise Diffusion.}} a) In vanilla diffusion models, the noise direction at each point along the ODE path points toward the final destination.
b) In stage-wise diffusion, the noise direction at each point is oriented to the endpoint of the current stage. Compared to traditional diffusion, this approach reduces the training difficulty as the target is much closer.}
    \label{fig:StageDiffusion}
\end{figure}
